LAraBench: Benchmarking Arabic AI with Large Language Models

Recent advancements in Large Language Models (LLMs) have significantly influenced the landscape of language and speech research. Despite this progress, these models lack specific benchmarking against state-of-the-art (SOTA) models tailored to particular languages and tasks. LAraBench addresses this gap for Arabic Natural Language Processing (NLP) and Speech Processing tasks, including sequence tagging and content classification across different domains. We utilized models such as GPT-3.5-turbo, GPT-4, BLOOMZ, Jais-13b-chat, Whisper, and USM, employing zero and few-shot learning techniques to tackle 33 distinct tasks across 61 publicly available datasets. This involved 98 experimental setups, encompassing ~296K data points, ~46 hours of speech, and 30 sentences for Text-to-Speech (TTS). This effort resulted in 330+ sets of experiments. Our analysis focused on measuring the performance gap between SOTA models and LLMs. The overarching trend observed was that SOTA models generally outperformed LLMs in zero-shot learning, with a few exceptions. Notably, larger computational models with few-shot learning techniques managed to reduce these performance gaps. Our findings provide valuable insights into the applicability of LLMs for Arabic NLP and speech processing tasks.

==> sections/dataset_old.tex <==
% \section{LLM Benchmark}
% \label{sec:benchmark}

% \subsection{Motivation}
% \label{ssec:motivation}


\section{Tasks and Datasets}
\label{sec:tasks_and_dataset}

The \arabench{} study was designed with an ambitious goal 
%to enable 
of empowering the research community and practitioners 
%to conduct 
 with the most comprehensive evaluation of LLMs for Arabic NLP and Speech tasks to date.
 % and, therefore, it assembled 
%the largest 
 % an extensive suite of test sets used by SOTA models. % needed for experimentation. 
 %Through this comprehensive evaluation, we seek to unravel the performance and capabilities of LLMs in tackling various Arabic NLP tasks. Our research paper promises to provide valuable insights and serve as a crucial reference for future advancements in Arabic NLP benchmarking. 
 It includes 61 publicly available datasets to support 9 task groups\footnote{%Our categorization is derived from the taxonomy of subareas within the field, as outlined in the list of tracks established by ACL 2022.
Our task categorization is derived from the taxonomy outlined in the list of tracks established by ACL 2022.} discussed below.
% Word Segmentation, Syntax and Information Extraction, Machine Translation, Sentiment, Stylistic and Emotion Analysis, News Categorization, Demographic Attributes prediction, Ethics and NLP, Semantics, Questions Answering and, Speech Processing. 
%In this section
We briefly describe each task and refer to Appendix~\ref{sec:appx-tasks-datasets} for a comprehensive description of tasks and datasets.
%Please refer to Table~\ref{} for a sample of tasks for each category and Appendix~\ref{sec:appx-tasks-datasets} for a more comprehensive table.  
 

% \todo[]{\maram{a chart and table summarizing all tasks + datasets used + datasets distribution will be useful here}}
% We organize the tasks into the following categories
% \begin{enumerate}
    % \item{Sequence Tagging/ Token classification / Core linguistics}: This category covers the following tasks:
    % \begin{itemize}

% \maram{I suggest we give an abbreviation in each task and subtask title here to make it easier to reference them later on in tables}

% \subsection{Sequence Tagging}
%\subsection{Word Segmentation, Syntax and Information Extraction}
\paragraph{Word Segmentation, Syntax and Information Extraction.}
This task group involves sequence tagging and sentence level classification. 
Sequence tagging tasks in NLP involve assigning labels or tags to individual elements within a sequence of text, e.g.,  Part-of-speech (POS) tagging.
We explore six such tasks:  i) word segmentation, ii) POS-tagging, iii) lemmatization, iv) diacritization, v) parsing, and vi) named-entity recognition (NER), using publicly available datasets (see Appendix~\ref{sec:appx-tasks-datasets}). 

We also include a dialect identification task (e.g., Egyptian dialect) since vocabulary, pronunciation, grammar, and idiomatic expressions vary across dialects. For our benchmarking we used QADI~\cite{abdelali-etal-2021-qadi} and ADI (in-house) datasets.

%Therefore, it is important to determine the specific dialect or regional variant of Arabic used in a given text or speech sample. 
% datasets such as: \citet{samih2017learning,darwish2018diacritization}.%, and vii) paraphrasing.

%\subsection{Machine Translation}
\paragraph{Machine Translation.}
Machine translation of Arabic language
%and dialects
 presents unique challenges due to morphological complexity %syntactic structure, ambiguity and polysemy,
and dialectal variations. %, that make it a harder task compared to other languages. 
 Addressing these challenges 
 requires advanced techniques, such as
 %comprehensive linguistic analysis, 
 domain adaptation,
 %context-aware models, 
  and effective handling of dialectal variations. %Researchers have developed a plethora of test-sets towards this goal. 
  We include AraBench \cite{sajjad2020arabench}, an extensive MT suite of data %offering 4 coarse, 15 fine-grained and 25 city-level dialect categories, belonging to 
 from diverse genres %, such as media, chat, religion and travel 
  and dialects. %Please refer to Table \ref{} in Appendix \ref{}.

% \subsection{Dialect Identification} 

% The dialectal identification problem in Arabic refers to the challenge of determining the specific dialect or regional variant of Arabic used in a given text or speech sample. Arabic encompasses numerous dialects (e.g., Egyptian) that vary significantly in terms of vocabulary, pronunciation, grammar, and idiomatic expressions. 
%Some well-known dialects include Egyptian Arabic, Levantine Arabic, Gulf Arabic, and Maghrebi Arabic. 
% For our benchmarking we used QADI~\cite{abdelali-etal-2021-qadi} and ADI (in-house) datasets.


%\subsection{Sentiment, Stylistic and Emotion Analysis}
\paragraph{Sentiment, Stylistic and Emotion Analysis.}

These tasks involve understanding and analyzing aspects of human expression and communication. Sentiment analysis involves classifying text as positive, neutral, or negative for each sentiment. Stylistic analysis characterizes author's writing style.%, tone, or intention
We benchmark Sentiment Analysis, Emotion Recognition, Stance Detection, and Sarcasm Detection with datasets from \citet{elmadany2018arsas}, \citet{mohammad2018semeval}, \citet{chouigui2017ant}, and \citet{abufarha-etal-2021-arsarcasm-v2}, respectively.

%\subsection{News Categorization}
\paragraph{News Categorization.}
This task involves classification of news articles into pre-defined categories or topics \cite{sebastiani2002machine}. This has been extended to cover categorization of tweets. 
We support benchmark evaluations using SANAD news article corpus~\cite{einea2019sanad} and ASND social media dataset~\cite{chowdhury2020improving}.
%, which encompasses data from various social media platforms such as Twitter, Facebook, and YouTube.

%\subsection{Demographic Attributes}
\paragraph{Demographic Attributes.}

Demographic information, including gender, age, and country of origin, hold significant value across various applications such as population analysis. %, personalized marketing, socio-cultural studies, and more. 
 %Governments, businesses, and organizations leverage demographic data to gain insights into their target audiences and effectively strategize for the future. 
 We include datasets that enable experimentation with tasks of identifying country, gender~\cite{mubarak2022arabgend} and location \cite{mubarak2021ul2c}.

%\subsection{Factuality, Disinformation and Harmful Content Detection}

\paragraph{Ethics and NLP: Factuality, Disinformation and Harmful Content Detection.}

Factuality, disinformation, and harmful content detection have emerged as critical areas within the field of NLP. 
%With %the rise of social media platforms and 
 %the rapid spread of information online, there is a pressing need to ensure accuracy and reliability of textual content. Detecting factuality helps combat the spread of misinformation, %disinformation, and fake news, 
  %while identifying harmful content protects users from exposure to offensive, or abusive material. 
  We support benchmarking of several \emph{detection} tasks, such as: i) Propaganda~\cite{alam2022overview}, ii) Check-worthiness~\cite{nakov2022overview}, iii) Claim~\cite{alam2020call2arms}, iv) Factuality using the datasets~\citet{baly-etal-2018-predicting,alam-etal-2021-fighting-covid,khouja-2020-stance}, v) Harmful content~\cite{nakov2022overview}, vi) Offensive language~\cite{zampieri2020semeval},  vii) Hate speech~\cite{mubarak2021adult}, and  viii) Spam~\cite{mubarak2020spam}.

  
  %namely: i) Subjectivity Identification based on the AraFacts dataset \cite{ali2021arafacts}, ii) Propaganda Detection using twitter multilabel and multiclass span level classification task \cite{alam2022overview}, iii) Check-worthiness detection using Arabic subset of CLEF2022 CheckThat Lab~\citep{nakov2022overview}, iv) Claim Detection using a multi-question annotation schema \citet{alam2020call2arms} and \citet{khouja-2020-stance}, v) Attention-worthiness detection also using the CLEF2022 CheckThatLab, vi) Factuality detection using the dataset developed by \citet{baly-etal-2018-predicting}, vii) Harmful Content Detection \cite{nakov2022overview}, viii) Offensive Language Detection ~\citep{zampieri2020semeval}, Hate Speech Detection \citep{mubarak2021adult}, and Spam Detection \cite{mubarak2020spam}.

\paragraph{Semantics.}
% \paragraph{Semantic Textual Similarity (STS)}
%\subsection{Semantic Textual Similarity (STS)}
This task group includes Semantic Textual Similarity (STS) and Natural Language Inference (NLI). 
% Semantic textual similarity is a measure used to 
% determine if two sentences are semantically equivalent. 
We benchmark STS using datasets from two research community tasks: SemEval-2017 focused on semantic similarity between Arabic and Arabic-English sentence pairs \cite{cer-etal-2017-semeval} and similarity in Arabic question pairs, as explored by \citet{seelawi2019nsurl}.
%\subsection{Natural Language Inference (NLI)}
% \paragraph{Natural Language Inference (NLI)}
% The XNLI task serves as a rigorous evaluation of the cross-lingual transfer capabilities of NLP models, assessing their ability to understand and reason in different languages within a multilingual context.
% For this study, 
For the XNLI task we used the translated version of Arabic from XNLI corpus~\cite{conneau2018xnli}. 
%\subsection{Question Answering (QA)}
\paragraph{Question Answering (QA).}
% Question Answering, also known as machine reading comprehension, focuses on answering questions in Arabic by leveraging a given text. In our study,
For the QA task, we employed included ARCD~\cite{mozannar2019neural}, MLQA~\cite{lewis2019mlqa}, TyDiQA~\cite{tydiqa}, and XQuAD~\cite{artetxe2019cross} datasets.
%, to assess the performance of question answering systems \cite{cite}

%\subsection{Speech Processing} 
\paragraph{Speech Processing.} 
We evaluate the large speech models on two tasks: speech recognition (ASR) and text-to-speech (TTS) synthesis. For ASR, we include datasets varying domain and dialects, e.g. MGB2~\cite{ali2016mgb}, QASR.CS~\cite{mubarak2021qasr} and ESCWA.CS~\cite{ali2021arabic}. For TTS, we evaluated with in-house 30 test sentences, covering diverse topics (e.g., education, health).
% Details in Table \ref{tab:datasets-speech}.

% such as broadcast (MSA and DA: MGB2,3 and 5), telephony (CallHomeEGY), meeting with code-switching (ESCWA.CS) among others (See \ref{tab:datasets-speech}). For TTS, we developed a test set with 30 sentences, covering diverse topics (e.g., education, health). 

% MGB2,3 and MGB5 along with other datasets such as ESCWA.CS~\cite{ali2021arabic} (See \ref{tab:datasets-speech}). For TTS, we developed a test set with 30 sentences, covering diverse topics (e.g., education, health). 
 % and QASR.CS~\cite{mubarak2021qasr}
%In the domain of speech processing, we conducted an evaluation of the performance of Language and Linguistics Models (LLMs) in two key tasks: speech recognition and text-to-speech synthesis. For speech recognition, we utilized a range of well-established datasets, including MGB2-5, ESCWA.CS, QASR.CS, DACS, and CallHome Egyptian \cite{cite}. In addition, we developed an in-house test dataset specifically for text-to-speech synthesis. This dataset, which is publicly available, consists of 20 sentences covering diverse topics such as psychology, education, and health. 


    

